Measurement of the ttbar production cross section in the tau+jets channel using the ATLAS detector

A measurement of the top quark pair production cross section in the final state with a hadronically decaying tau lepton and jets is presented. The analysis is based on proton-proton collision data recorded by the ATLAS experiment at the LHC, with a centre-of-mass energy of 7 TeV. The data sample corresponds to an integrated luminosity of 1.67 inverse femtobarns. The cross section is measured to be 194 +/- 18 (stat.) +/- 46 (syst.) pb and is in agreement with other measurements and with the Standard Model prediction.

==> commands.tex <==
\RequirePackage{xspace}

\def\metsig      {\ensuremath{S_{E_{\mathrm{T}}^{\mathrm{miss}}}}\xspace}
\def\sumet       {\ensuremath{\Sigma\,E_{\mathrm{T}}}\xspace}
\def\lumiunits   {\ensuremath{\mathrm{cm^{-2} s^{-1}}}\xspace}
\def\tauhad      {\ensuremath{\tau_{\mathrm{had}}}\xspace}
\def\LumiUsed    {{\bf XXX}~\lumiunits}
\def\DeltaR      {\ensuremath{\mathrm{\Delta} R}\xspace}
\def\mytau       {\ensuremath{\tau}\xspace}
\def\ntrack      {\ensuremath{n_{\mathrm{track}}}\xspace}
\def\numTrack    {\emph{numTrack}\xspace}
\def\nTrackKt    {\emph{nTrackKt}\xspace}
\def\ktthresh    {\ensuremath{kt_{thresh}}\xspace}
\def\ptcand      {\ensuremath{\mathrm{p_{\mathrm{T}}^{cand}}}\xspace}
\def\qcd         {\emph{gluon-jet}\xspace}
\def\comb        {\emph{quark-jet}\xspace}
\def\tauele      {\emph{tau/electron}\xspace}
\def\ntrue       {\ensuremath{\mathrm{n_{true}}}}
\def\nfit        {\ensuremath{\mathrm{n_{fit}}}}
\def\sigstat     {\ensuremath{\mathrm{\sigma_{stat}}}}
\def\sigsys      {\ensuremath{\mathrm{\sigma_{sys}}}}

\def\wtaunu      {\ensuremath{W\rightarrow\tau\nu_{\tau}}\xspace}
\def\ztautau     {\ensuremath{Z\rightarrow\tau\tau}\xspace}    
\def\abseta      {\ensuremath{|\,\eta\,|}\xspace}

\makeatletter
\newcommand\wrapfill{\par
  \ifx\parshape\WF@fudgeparshape
  \nobreak
  \vskip-\baselineskip
  \vskip\c@WF@wrappedlines\baselineskip
  \allowbreak
  \WFclear
  \fi
}
\makeatother 

% renew used shortcuts to add \xspace
\renewcommand{\pt}{\ensuremath{p_{\mathrm{T}}}\xspace}
\renewcommand{\met}{\ensuremath{E_{\mathrm{T}}^{\mathrm{miss}}}\xspace}
\renewcommand{\ttbar}{\ensuremath{t\bar{t}}\xspace}

